An energy-based discontinuous Galerkin method for the wave equation with advection

An energy-based discontinuous Galerkin method for the advective wave equation is proposed and analyzed. Energy-conserving or energy-dissipating methods follow from simple, mesh-independent choices of the inter-element fluxes, and both subsonic and supersonic advection is allowed. Error estimates in the energy norm are established, and numerical experiments on structured grids display optimal convergence in the $L^2$ norm for upwind fluxes. The method generalizes earlier work on energy-based discontinuous Galerkin methods for second order wave equations which was restricted to energy forms written as a simple sum of kinetic and potential energy.

==> error_estimates_old.tex <==
%!TEX root = wave_backgroundflow.tex
\section{Error estimates in the energy norm}\label{energyerr}
We define the errors by
\bd %\label{error_u_v}
e_u = u - u^h, \ \  e_v = v - v^h,
\ed
and let
\bd %\label{D_definition}
\mathbf{D}^h = (e_u, e_v).
\ed
Note the fundamental Galerkin orthogonality relation:
\bd % \label{DG_orthogonality_relation}
\mathcal{B}(\mathbf{\Phi}, \mathbf{D}^h) = 0.
\ed

To proceed we follow the standard approach of comparing $(u^h, v^h)$ to an arbitrary polynomial $(\tilde{u}^h, \tilde{v}^h)\in\mathcal{P}^{q,s,m}$. we define the differences
\bd
\tilde{e}_u = \tilde{u}^h - u^h, 
\ \ \tilde{e}_v = \tilde{v}^h - v^h, 
\ \  \delta_u = \tilde{u}^h - u, 
\ \  \delta_v = \tilde{v}^h - v,
\ed
and let
\bd
\tilde{\mathbf{D}}^h = (\tilde{e}_u, \tilde{e}_v)\in\mathcal{P}^{q,s,m}, 
\ \  \tilde{\mathbf{D}}_0^h = (\tilde{e}_u, \tilde{e}_v, 0)\in\mathcal{P}^{q,s,m}\times\mathcal{N}, 
\ \  \mathbf{\Delta}^h = (\delta_u, \delta_v).
\ed
Then, since $\mathbf{D}^h = \tilde{\mathbf{D}}^h - \mathbf{\Delta}^h$, we have the error equation
\bd % \label{equality_10}
\mathcal{B}(\tilde{\mathbf{D}}_0^h, \tilde{\mathbf{D}}^h)=\mathcal{B}(\tilde{\mathbf{D}}_0^h, \mathbf{\Delta}^h).
\ed
Finally, define the energy of $\tilde{\mathbf{D}}^h$ by
\bd %\label{error_energy}
\mathcal{E}^h = \frac{1}{2}\sum_{j}\int_{\Omega_j}\tilde{e}_v^2 + c^2|\nabla\tilde{e}_u|^2.
\ed
Then repeating the arguments which led to (\ref{derivative_discrete_energy_all}), we derive:
\begin{multline} \label{derivative_error_energy}
\frac{d\mathcal{E}^h}{dt} = 
\mathcal{B}(\tilde{D}_0^h, \mathbf{\Delta}^h) \\
- \sum_j\int_{F_j} \Big[ c^{2}\eta[[\nabla \tilde{e}_u]]^2
 + c^{2}\beta\big|[[\tilde{e}_v]]\big|^2
  - c^{2}\beta[[\tilde{e}_v]]\cdot\big(\nabla\tilde{e}_{u1}(\mathbf{w}\cdot\mathbf{n}_1)  \\
 +\nabla \tilde{e}_{u2}(\mathbf{w}\cdot\mathbf{n}_2)\big)
  -\eta [[\nabla \tilde{e}_u]][[\tilde{e}_v]]\cdot\mathbf{w} \Big] \\
+ \sum_j\int_{B_{j_I}} 
\Big[\frac{c^2\mathbf{w}\cdot\mathbf{n}}{2} \arrowvert (\nabla\tilde{e}_u)_{\tau} \arrowvert^2 
 + \frac{c^2\mathbf{w}\cdot\mathbf{n}}{2}(\nabla\tilde{e}_u\cdot\mathbf{n})^2 
+ \Big(\frac{\mathbf{w}\cdot\mathbf{n}}{2}
+\frac{(\mathbf{w}\cdot\mathbf{n})^2-c^2}{\xi-\mathbf{w}\cdot\mathbf{n}}\Big)(\tilde{e}_v)^2 \\
 + \frac{(c^2-\xi\mathbf{w}\cdot\mathbf{n})\mathbf{w}\cdot\mathbf{n}}{\xi-\mathbf{w}\cdot\mathbf{n}}(\nabla \tilde{e}_u\cdot\mathbf{n})\tilde{e}_v \Big] 
+ \sum_j\int_{B_{j_O}} \Big[ -\frac{c^2}{2} \arrowvert (\nabla \tilde{e}_u)_{\tau}\arrowvert^2\mathbf{w}\cdot\mathbf{n}   \\
  + (\frac{c^2}{2\xi}+\frac{\xi}{2})(\nabla \tilde{e}_u\cdot\mathbf{n})\tilde{e}_v\mathbf{w}\cdot\mathbf{n}
 -\frac{c^2\xi}{2}(\nabla \tilde{e}_u\cdot\mathbf{n})^2-\frac{c^2}{2\xi}(\tilde{e}_v)^2 \Big].  
\end{multline}

We now must choose $(\tilde{u}^h, \tilde{v}^h)$ to achieve an acceptable error estimate. In what follows we will assume for simplicity that $(u^h, v^h) = (\tilde{u}^h, \tilde{v}^h)$ at $t = 0$. We note that in the numerical experiments we found it beneficial to subtract off a function satisfying the initial conditions, thus solving a forced equation with zero initial data. On $\Omega_j$ we impose for all times $t$ and $(\phi_u, \phi_v)\in\mathcal{P}^{q,s,m}$,
\be \label{restriction_polynomials}
\int_{\Omega_j}\nabla\phi_u\cdot\nabla\delta_u = \int_{\Omega_j}\phi_v\delta_v = \int_{\Omega_j}\delta_u = 0 .
\ee
Then, integrating by parts, we derive the following expression for $\mathcal{B}(\tilde{\mathbf{D}}_0^h, \mathbf{\Delta}^h)$: 
\begin{multline*} %\label{B_definition_1}
\mathcal{B}(\tilde{\mathbf{D}}_0^h, \mathbf{\Delta}^h) = \sum_j\int_{\Omega_j} \Big[ c^2\nabla\tilde{e}_u\cdot\nabla(\frac{\partial \delta_u}{\partial t}) 
 -c^2\nabla^2\tilde{e}_u\mathbf{w}\cdot\nabla\delta_u 
  + c^2\nabla^2\tilde{e}_u\delta_v + \tilde{e}_v(\frac{\partial \delta_v}{\partial t})  \\
- \mathbf{w}\cdot\nabla\tilde{e}_v\delta_v 
+ c^2\nabla\tilde{e}_v\cdot\nabla\delta_u \Big]
- \sum_j \int_{\partial\Omega_j} \Big[ -c^2\nabla\tilde{e}_u\cdot\mathbf{n}\nabla\delta_u\cdot\mathbf{w}  
+ c^2\delta_v^*\nabla\tilde{e}_u\cdot\mathbf{n} \\
+ c^2\tilde{e}_v\nabla\delta_u^*\cdot\mathbf{n} 
- c^2\nabla\tilde{e}_u\cdot(\nabla\delta^*_u-\nabla\delta_u)\mathbf{w}\cdot\mathbf{n}
- \delta_v^*\tilde{e}_v\mathbf{w}\cdot\mathbf{n} \Big],
\end{multline*}
now  we can rewrite the volume integral $\int_{\Omega_j}\nabla^2\tilde{e}_u\mathbf{w}\cdot\nabla\delta_u$ as,
\bd %\label{equality_11}
\int_{\Omega_j}\nabla^2\tilde{e}_u\mathbf{w}\cdot\nabla\delta_u = \int_{\Omega_j}\big(\nabla(\mathbf{w}\cdot\nabla\tilde{e}_u)+\nabla\times(\mathbf{w}\times\nabla\tilde{e}_u)\big)\cdot\nabla\delta_u,
\ed
then invoking (\ref{restriction_polynomials}) the volume integrals in $\mathcal{B}(\tilde{\mathbf{D}}_0^h, \mathbf{\Delta}^h)$ will vanish and we can simplify $\mathcal{B}(\tilde{\mathbf{D}}_0^h, \mathbf{\Delta}^h)$ to
\begin{multline} \label{B_definition_2}
\mathcal{B}(\tilde{\mathbf{D}}_0^h, \mathbf{\Delta}^h) =
- \sum_j \int_{\partial\Omega_j}c^2\big((\mathbf{w}\times\nabla\tilde{e}_u)\times\nabla\delta_u\big)\cdot\mathbf{n}
-c^2\nabla\tilde{e}_u\cdot\mathbf{n}\nabla\delta_u\cdot\mathbf{w}\\
+ c^2\delta_v^*\nabla\tilde{e}_u\cdot\mathbf{n} + c^2\tilde{e}_v\nabla\delta_u^*\cdot\mathbf{n} 
-c^2\nabla\tilde{e}_u\cdot(\nabla\delta^*_u-\nabla\delta_u)\mathbf{w}\cdot\mathbf{n}
- \delta_v^*\tilde{e}_v\mathbf{w}\cdot\mathbf{n}\\
=- \sum_j \int_{\partial\Omega_j}c^2\big(-(\nabla\delta_u\cdot\nabla\tilde{e}_u)\mathbf{w}\cdot\mathbf{n}
+\nabla\tilde{e}_u\cdot\mathbf{n}\nabla\delta_u\cdot\mathbf{w}\big)
-c^2\nabla\tilde{e}_u\cdot\mathbf{n}\nabla\delta_u\cdot\mathbf{w} \\
+ c^2\delta_v^*\nabla\tilde{e}_u\cdot\mathbf{n} 
+ c^2\tilde{e}_v\nabla\delta_u^*\cdot\mathbf{n} 
-c^2\nabla\tilde{e}_u\cdot(\nabla\delta^*_u-\nabla\delta_u)\mathbf{w}\cdot\mathbf{n}- \delta_v^*\tilde{e}_v\mathbf{w}\cdot\mathbf{n}\\
=- \sum_j \int_{\partial\Omega_j}c^2\delta_v^*\nabla\tilde{e}_u\cdot\mathbf{n} - \delta_v^* \tilde{e}_v\mathbf{w}\cdot\mathbf{n}+ c^2\tilde{e}_v\nabla\delta_u^*\cdot\mathbf{n} - c^2\nabla\tilde{e}_u\cdot\nabla\delta_u^*\mathbf{w}\cdot\mathbf{n} .  
\end{multline}

Combining contributions from neighboring elements we then have 
\begin{multline*} %\label{B_definition_3}
\mathcal{B}(\tilde{\mathbf{D}}_0^h, \mathbf{\Delta}^h) 
= - \sum_j \int_{F_j} \Big[ c^2[[\nabla\tilde{e}_u]]\delta_v^* 
-[[\tilde{e}_v]]\delta_v^*\cdot\mathbf{w}
+ c^2[[\tilde{e}_v]]\cdot\nabla\delta_u^*\\
- c^2\nabla\tilde{e}_{u1}\cdot\nabla\delta_u^*\mathbf{w}\cdot\mathbf{n}_1
 - c^2\nabla\tilde{e}_{u2}\cdot\nabla\delta_u^*\mathbf{w}\cdot\mathbf{n}_2 \Big]\\
  - \sum_j \int_{B_j} \Big[ c^2\delta_v^*\nabla\tilde{e}_u\cdot\mathbf{n}
   - \delta_v^* \tilde{e}_v\mathbf{w}\cdot\mathbf{n}
   + c^2\tilde{e}_v\nabla\delta_u^*\cdot\mathbf{n} 
  - c^2\nabla\tilde{e}_u\cdot\nabla\delta_u^*\mathbf{w}\cdot\mathbf{n} \Big].
\end{multline*}
Here we have introduced the fluxes $\delta_v^*$, $\nabla\delta_u^*$ built from $\delta_v$, $\nabla\delta_u$ according to the specification in Section \ref{fluxes}. In what follows, $C$ will be a constant independent of the solution and the element diameter $h$ for a shape-regular mesh. Here $||\cdot||$ denotes a Sobolev norm and $|\cdot|$ denotes the associated seminorm. We then have the following error estimate.
\begin{theorem}
Let $\bar{q} = \min(q-1,s)$. Then there exist numbers $C_0$, $C_1$ depending only on $s$, $q$ and the shape-regularity of the mesh, such that for smooth solutions $u$, $v$ and time $T$
\begin{multline*}
||\nabla e_{u}(\cdot,T)||_{{L^2}(\Omega)}^2 + ||e_v(\cdot,T)||_{L^2(\Omega)}^2 \\
\leq (C_0T + C_1T^2)\max_{t\leq T}\Big[h^{2\theta}\big(|u(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2 + |v(\cdot,t)|_{H^{\bar{q}+1}(\Omega)}^2\big)\Big],
\end{multline*}  
where
\begin{eqnarray*}
 \theta = \left\{
\begin{array}{ll}
\bar{q},   \ \ \ \ \ \ \ \  \ \ \  \beta,\eta\geq0, \ \ |{\bf w}\cdot{\bf n}| \leq \frac{2c^2\xi}{c^2+\xi^2},\\
\bar{q}+\frac{1}{2},\ \ \ \ \  \ \beta,\eta > 0, \ \ |{\bf w}\cdot{\bf n}|\leq \frac{2c^2\xi}{c^2+\xi^2}.
\end{array}
\right.
\end{eqnarray*}
\end{theorem}

\begin{proof}
From the Bramble-Hilbert lemma (e.g. \ci{Ciarlet}), we have for $\bar{q}=\min (q-1,s)$ 
\begin{align*} 
 \| \delta_v \|_{L^2(\Omega)}^2 + \|\nabla\delta_u\|_{L^2(\Omega)}^2
 &\leq Ch^{2\bar{q}+2}\left(|u(\cdot,t)|_{H^{\bar{q}+2}}^2 + |v(\cdot,t)|_{H^{\bar{q}+1}(\Omega)}^2\right),\\
 \|\frac{\partial\delta_v}{\partial t}\|_{L^2(\Omega)}^2 
& \leq  Ch^{2s+2} \left| \frac{\partial v(\cdot,t)}{\partial t} \right|_{H^{s+1}(\Omega)}^2,\\
 \|\delta_v^*\|_{L^2(\partial\Omega)}^2 + \|\nabla\delta_{u}^*\cdot\mathbf{n} \|_{L^2(\partial\Omega)}^2 
 & \leq  Ch^{2\bar{q}+1}\left(|u(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2 + |v(\cdot,t)|_{H^{\bar{q}+1}(\Omega)}^2\right), \\%\\ \label{inequality_10} \\
 \|\tilde{e}_v\|_{L^2(\partial\Omega)}^2 + \|\nabla\tilde{e}_u\cdot\mathbf{n}\|_{L^2(\partial\Omega)}^2 
 & \leq  Ch^{-1}\left(\|\tilde{e}_v\|_{L^2(\Omega)}^2 + \|\nabla\tilde{e}_u\|_{L^2(\Omega)}^2\right). %\label{inequality_11}
\end{align*}
First, consider the case where $\beta = 0$ or $\eta = 0$. From the condition (\ref{bound_w_1}) we conclude that the time derivative of the error energy satisfies 
\bd
\frac{d\mathcal{E}^h}{dt} \leq \mathcal{B}(\tilde{\mathbf{D}}_0^h, \mathbf{\Delta}^h).
\ed
 Now, by the Cauchy-Schwarz inequality we have 
\begin{multline*} 
\mathcal{B}(\tilde{\mathbf{D}}_0^h, \mathbf{\Delta}^h)  
\leq  C\sum_{j}\|\nabla\tilde{e}_u\cdot\mathbf{n}\|_{L^2(\partial\Omega_j)}\|\delta^*_v\|_{L^2(\partial\Omega_j)} 
+\|\tilde{e}_v\|_{L^2(\partial\Omega_j)}\|\nabla\delta^*_u\cdot \mathbf{n}\|_{L^2(\partial\Omega_j)}\\
+\|\nabla\tilde{e}_u\|_{L^2(\partial\Omega_j)}\|\nabla\delta^*_u\|_{L^2(\partial\Omega_j)} 
+\|\delta^*_v\|_{L^2(\partial\Omega_j)}\|\tilde{e}_v\|_{L^2(\partial\Omega_j)} \\
\leq C\sqrt{\mathcal{E}^h}h^{\bar{q}}(|u(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}
+|v(\cdot,t)|_{H^{\bar{q}+1}(\Omega)}).  
\end{multline*}
Then a direct integration in time combined with the assumption that $(\tilde{e}_u, \tilde{e}_v) = 0$ at $t = 0$ gives us
\bd % \label{error_bound_1}
\mathcal{E}^h(T) \leq CT^2 \max_{t\leq T} h^{2\bar{q}}\left(|u(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2+|v(\cdot,t)|_{H^{\bar{q}+1}(\Omega)}^2\right).
\ed 
For dissipative fluxes, $\beta$, $\eta > 0$, we can improve the estimates. For the boundaries of the inter-elements the contribution is
\begin{multline*}
\Theta_1 = -\sum_j \int_{F_j} \Big[ c^2[[\nabla\tilde{e}_u]]\delta_v^* 
 -[[\tilde{e}_v]]\delta_v^*\cdot\mathbf{w}
 + c^2[[\tilde{e}_v]]\cdot\nabla\delta_u^*
 - c^2\nabla\tilde{e}_{u1}\cdot\nabla\delta_u^*\mathbf{w}\cdot\mathbf{n}_1   \\
   - c^2\nabla\tilde{e}_{u2}\cdot\nabla\delta_u^*\mathbf{w}\cdot\mathbf{n}_2 \Big] 
  - \sum_j\int_{F_j} \Big[ c^{2}\eta[[\nabla\tilde{e}_u]]^2 
  + c^{2}\beta\big|[[\tilde{e}_v]]\big|^2  \\
   -c^{2}\beta[[\tilde{e}_v]]\cdot\big(\nabla\tilde{e}_{u1} 
(\mathbf{w}\cdot\mathbf{n}_1)
+\nabla \tilde{e}_{u2}(\mathbf{w}\cdot\mathbf{n}_2)\big)
-\eta [[\nabla\tilde{e}_u]][[\tilde{e}_v]]\cdot\mathbf{w} \Big], 
\end{multline*}
resulting in
\begin{multline} \label{inequality_12}
\Theta_1 \leq  C\sum_j \Big(\|\delta_v^*\|_{L^2(F_j)}^2 + \|\nabla\delta_u^*\|_{L^2(F_j)}^2\Big)  \\
 \leq  Ch^{2\bar{q}+1}\Big(|u(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2 + |v(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2\Big),
\end{multline}
on the physical boundaries, by using the fact 
\[
\nabla \tilde{e}_u\cdot\nabla\delta_u^* = (\nabla\tilde{e}_u\cdot{\bf n})(\nabla\delta_u^*\cdot{\bf n}) + (\nabla\tilde{e}_u)_\tau\cdot(\nabla\delta_u^*)_\tau,
\]
at inflow we have
\begin{multline*} %\label{inequality_13}
\Theta_2 %=  - \sum_j \int_{B_{j_I}} \Big[ c^2\delta_v^*\nabla\tilde{e}_u\cdot\mathbf{n} 
 %- \delta_v^* \tilde{e}_v\mathbf{w}\cdot\mathbf{n}
 %+ c^2\tilde{e}_v\nabla\delta_u^*\cdot\mathbf{n} 
 %- c^2\nabla\tilde{e}_u\cdot\nabla\delta_u^*\mathbf{w}\cdot\mathbf{n} \Big] \\
% +\sum_j\int_{B_{j_I}} \Big[ \frac{c^2\mathbf{w}\cdot\mathbf{n}}{2}\arrowvert (\nabla\tilde{e}_u)_{\tau}\arrowvert^2
% + \frac{c^2\mathbf{w}\cdot\mathbf{n}}{2}(\nabla\tilde{e}_u\cdot\mathbf{n})^2 
% + \Big(\frac{\mathbf{w}\cdot\mathbf{n}}{2}
 %+\frac{(\mathbf{w}\cdot\mathbf{n})^2-c^2}{\xi-\mathbf{w}\cdot\mathbf{n}}\Big) \cdot (\tilde{e}_v)^2  \\
%+ \frac{(c^2-\xi\mathbf{w}\cdot\mathbf{n})\mathbf{w}\cdot\mathbf{n}}{\xi-\mathbf{w}\cdot\mathbf{n}}(\nabla \tilde{e}_u\cdot\mathbf{n})\tilde{e}_v \Big] \\
 = - \sum_j \int_{B_{j_I}} \Big[ c^2\delta_v^*\nabla\tilde{e}_u\cdot\mathbf{n} 
 - \delta_v^* \tilde{e}_v\mathbf{w}\cdot\mathbf{n}
 + c^2\tilde{e}_v\nabla\delta_u^*\cdot\mathbf{n} 
 - c^2(\nabla\tilde{e}_u\cdot\mathbf{n})(\nabla\delta_u^*\cdot\mathbf{n})\mathbf{w}\cdot\mathbf{n}   \\
  -c^2(\nabla\tilde{e}_u)_{\tau} \cdot (\nabla\delta_u^*)_{\tau} \mathbf{w}\cdot\mathbf{n} \Big] 
  +\sum_j\int_{B_{j_I}} \Big[ \frac{c^2\mathbf{w}\cdot\mathbf{n}}{2} \arrowvert (\nabla\tilde{e}_u)_{\tau}\arrowvert^2 
+ \frac{c^2\mathbf{w}\cdot\mathbf{n}}{2}(\nabla\tilde{e}_u\cdot\mathbf{n})^2  \\
  + \Big(\frac{\mathbf{w}\cdot\mathbf{n}}{2}
  +\frac{(\mathbf{w}\cdot\mathbf{n})^2-c^2}{\xi-\mathbf{w}\cdot\mathbf{n}}\Big) (\tilde{e}_v)^2
  + \frac{(c^2-\xi\mathbf{w}\cdot\mathbf{n})\mathbf{w}\cdot\mathbf{n}}{\xi-\mathbf{w}\cdot\mathbf{n}}(\nabla \tilde{e}_u\cdot\mathbf{n})\tilde{e}_v \Big]. 
  \end{multline*}
Thus
\bd% egin{multline*}  
\Theta _2 
 \leq  C\sum_j \Big(\|\delta_v^*\|_{L^2(B_{j_I})}^2 
+ \|\nabla\delta_u^*\|_{L^2(B_{j_I})}^2\Big)
 \leq  Ch^{2\bar{q}+1}\Big(|u(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2 
+ |v(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2\Big). 
\ed%nd{multline*}

Similarly, on the outflow boundaries we obtain that
\begin{multline*} % \label{inequality_14}
\Theta_3 %=  - \sum_j \int_{B_{j_O}} c^2\delta_v^*\nabla\tilde{e}_u\cdot\mathbf{n} 
 %- \delta_v^* \tilde{e}_v\mathbf{w}\cdot\mathbf{n} 
 %+ c^2\tilde{e}_v\nabla\delta_u^*\cdot\mathbf{n} 
 %- c^2\nabla\tilde{e}_u\cdot\nabla\delta_u^*\mathbf{w}\cdot\mathbf{n}  \\ 
 %+ \sum_j\int_{B_{j_O}}  
%-\frac{c^2}{2}\arrowvert (\nabla \tilde{e}_u)_{\tau}\arrowvert^2\mathbf{w}\cdot\mathbf{n}
%+\left(\frac{c^2}{2\xi}+\frac{\xi}{2}\right)(\nabla \tilde{e}_u\cdot\mathbf{n})\tilde{e}_v\mathbf{w}\cdot\mathbf{n}
%-\frac{c^2\xi}{2}(\nabla \tilde{e}_u\cdot\mathbf{n})^2
%-\frac{c^2}{2\xi}(\tilde{e}_v)^2 \\
  =  - \sum_j \int_{B_{j_O}} \Big[ c^2\delta_v^*\nabla\tilde{e}_u\cdot\mathbf{n} 
  - \delta_v^* \tilde{e}_v\mathbf{w}\cdot\mathbf{n}
  + c^2\tilde{e}_v\nabla\delta_u^*\cdot\mathbf{n} 
  - c^2(\nabla\tilde{e}_u\cdot\mathbf{n})(\nabla\delta_u^*\cdot\mathbf{n})\mathbf{w}\cdot\mathbf{n}   \\
  - c^2(\nabla\tilde{e}_u)_{\tau} \cdot (\nabla\delta_u^*)_{\tau} \mathbf{w}\cdot\mathbf{n} \Big] 
 + \sum_j\int_{B_{j_O}} \Big[ -\frac{c^2}{2} \arrowvert (\nabla \tilde{e}_u)_{\tau} \arrowvert^2\mathbf{w}\cdot\mathbf{n}   \\
  +(\frac{c^2}{2\xi}+\frac{\xi}{2}) (\nabla \tilde{e}_u\cdot\mathbf{n})\tilde{e}_v\mathbf{w}\cdot\mathbf{n}
 - \frac{c^2\xi}{2}(\nabla \tilde{e}_u\cdot\mathbf{n})^2
 - \frac{c^2}{2\xi}(\tilde{e}_v)^2 \Big].
 \end{multline*}
Then
\begin{multline} \label{inequality_14}
\Theta_3  \leq  C\sum_j \Big[ \|\delta_v^*\|_{L^2(B_{j_O})}^2 
 + \|\nabla\delta_u^*\|_{L^2(B_{j_O})}^2\Big] \\
 \leq  Ch^{2\bar{q}+1}\Big[|u(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2 
 + |v(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2\Big].
\end{multline}
Combining (\ref{derivative_error_energy}) with (\ref{inequality_12})-(\ref{inequality_14}) yields 
\bd%e  \label{error_bound_2}
\mathcal{E}^h(T) \leq CT \max_{t\leq T} h^{2\bar{q}+1}(|u(\cdot,t)|_{H^{\bar{q}+2}(\Omega)}^2+|v(\cdot,t)|_{H^{\bar{q}+1}(\Omega)}^2).
\ed%e
\end{proof}

\begin{rem}
A similar analysis yields the same results in the presence of supersonic boundaries, $\arrowvert \mathbf{w} \cdot \mathbf{n} \arrowvert > c$.
\end{rem} 


==> manuscript_tables/center_dbc_2d.tex <==
\newcommand*\centerdbctwod{
\begin{table}
\footnotesize
\begin{center}
  \begin{tabular}{|c|c c c c c c|}
  \hline
{Degree (q) of approx. of u and v~~~~~~}  & 1 & 2 & 3 & 4 & 5 & 6 \\
\hline
{Rate fit u $(w_{x}=0.5,w_{y}=0.5,c=1)$}&1.3563& 2.1926 & 4.1572 & 4.1590 & 6.0963 & 6.1160 \\
  {Rate fit v $(w_{x}=0.5,w_{y}=0.5,c=1)$}&0.4475 & 1.0069 & 2.8687 & 3.0257 & 4.9507 & 5.0039 \\
  \cline{1-7}
  {Rate fit u $(w_{x}=1,w_{y}=1,c=1)$~~~~~}&1.6394 & 3.0219 & 4.0026& 4.9804 & 5.9908 & 6.9683 \\
  {Rate fit v $(w_{x}=1,w_{y}=1,c=1)$~~~~~}
  &0.6009 & 1.9888 & 2.9491 & 4.0070 & 4.9718 & 5.9850  \\
  \cline{1-7}
\end{tabular}
\end{center}
\caption{\scriptsize{linear regression estimates the convergent rate of $u$ and $v$ in $2d$ with C.-flux for Dirichlet boundary condition on inflow boundaries, radiation boundary condition on outflow boundaries and $q_{x} = q_{y} = q$.}}
\label{R_Center_full_LR2}
\end{table}
}


==> modal_formulation.tex <==
%!TEX root = wave_backgroundflow.tex
\subsection{Modal formulation}
Considering 1d dimension to be an example, assume the computational domain has been discretized by a uniform grid $x_0, \cdots, x_i, x_{i+1}, \cdots x_{n}$ with spacing $h$. Let $x_{i+\frac{1}{2}} = (x_i + x_{i+1})/2$, then the mapping $z = \frac{2}{h}(x - x_{i+\frac{1}{2}})$ takes element $\Omega_{i} = (x_{i}, x_{i+1})$ to the reference element $\Omega_R = (-1, 1)$, where we expand the displacement $u^{h}$ and the material velocity $v^{h}$ in basis functions:
\begin{eqnarray}
    u^h(x,t) = \sum_{k=0}^{s}\hat{u}_{k}(t)\phi_k(x),\label{approximation_u}\\
    v^h(x,t) = \sum_{k=0}^{q}\hat{v}_{k}(t)\psi_k(x).\label{approximation_v}
\end{eqnarray}
It is convenient to arrange the expansion coefficients into $\hat{\textbf{u}} = [\hat{u}_{0}^h, \hat{u}_{1}^h, \cdots, \hat{u}_{s}^h]^{T}$ and $\hat{v} = [\hat{v}_{0}^h, \hat{v}_{1}^h, \cdots, \hat{v}_{q}^h]^{T}$, then the discrete version of (\ref{v_DG_use}) on an element can then be written as
\begin{eqnarray}\label{discrete_form_u}
    M^{v}\hat{\textbf{v}}^{'}(t) + G^{v}\hat{\textbf{v}}(t) + S^{u}\hat{\textbf{u}}(t) = \mathcal{F}^v.
\end{eqnarray}
Besides, the extra equation (\ref{extra_equation_u}) and the variational equation (\ref{u_DG_use}) can also be written into the system
\begin{eqnarray}\label{discrete_form_v}
    M^{u}\hat{\textbf{u}}^{'}(t) + G^{u}\hat{\textbf{u}}(t) + S^{v}\hat{\textbf{v}}(t) = \mathcal{F}^u.
\end{eqnarray}
where the exact expressions for the mass $(M^{u}, M^{v})$, stiffness $(S^{u}, S^{v})$ matrices and $G^u$, $G^v$ can be found in Appendix A. Here, we use Legendre polynomials as the basis and trial functions. For higher dimension spaces, we formulate the model formulation by the same idea with 1d case, and we choose the tensor product of Legendre polynomials to be basis functions of higher dimensions.

